On the Closed Form Expression of Elementary Symmetric Polynomials and the Inverse of Vandermonde Matrix

Inverse Vandermonde matrix calculation is a long-standing problem to solve nonsingular linear system $Vc=b$ where the rows of a square matrix $V$ are constructed by progression of the power polynomials. It has many applications in scientific computing including interpolation, super-resolution, and construction of special matrices applied in cryptography. Despite its numerous applications, the matrix is highly ill-conditioned where specialized treatments are considered for approximation such as conversion to Cauchy matrix, spectral decomposition, and algorithmic tailoring of the numerical solutions. In this paper, we propose a generalized algorithm that takes arbitrary pairwise (non-repetitive) sample nodes for solving inverse Vandermonde matrix. This is done in two steps: first, a highly balanced recursive algorithm is introduced with $\mathcal{O}(N)$ complexity to solve the combinatorics summation of the elementary symmetric polynomials; and second, a closed-form solution is tailored for inverse Vandermonde where the matrix' elements utilize this recursive summation for the inverse calculations. The numerical stability and accuracy of the proposed inverse method is analyzed through the spectral decomposition of the Frobenius companion matrix that associates with the corresponding Vandermonde matrix. The results show significant improvement over the state-of-the-art solutions using specific nodes such as $N$th roots of unity defined on the complex plane. A basic application in one dimensional interpolation problem is considered to demonstrate the utility of the proposed method for super-resolved signals.

==> arxiv submission/vander_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{cite}
\usepackage{graphicx,epstopdf,diagbox,multirow} % <- Preamble 
\usepackage[caption=false]{subfig}
\usepackage{rotating}


\makeatletter
\def\hlinewd#1{%
  \noalign{\ifnum0=`}\fi\hrule \@height #1 \futurelet
   \reserved@a\@xhline}

\newenvironment{conditions}
  {\par\vspace{\abovedisplayskip}\noindent\begin{tabular}{>{$}l<{$} @{${}={}$} l}}
  {\end{tabular}\par\vspace{\belowdisplayskip}}
  \newcounter{para}
\newcommand\mypara[1]{\par\refstepcounter{para}\textit{\thepara)\space#1\space}}
% Information that is shared between the article and the supplement
% (title and author information, macros, packages, etc.) goes into
% ex_shared.tex. If there is no supplement, this file can be included
% directly.

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\expnumber}[2]{{#1}\mathrm{e}{#2}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Elementary Symmetric Polynomials and Inverse of Vandermonde}{M. S. Hosseini, A. Chen, and K. N. Plataniotis}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{On the Closed Form Expression of Elementary Symmetric Polynomials and the Inverse of Vandermonde Matrix}

% Authors: full names plus addresses.
\author{Mahdi S. Hosseini\thanks{The Edward S. Rogers Sr. Department of Electrical \& Computer Engineering , University of Toronto, ON M5S 3G4, Ontario, Canada (\email{mahdi.hosseini@mail.utoronto.ca}, \email{lixiang.chen@mail.utoronto.ca}, \email{kostas@ece.utoronto.ca}).}
\and Alfred Chen\footnotemark[1]
\and Konstantinos N. Plataniotis\footnotemark[1]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

